ACWM-Phys: Investigating Generalized Physical Interaction in Action-Conditioned Video World Models

Action-conditioned world models (ACWMs) have shown strong promise for video prediction and decision-making. However, existing benchmarks are largely restricted to egocentric navigation or narrow, task-specific robotics datasets, offering only limited coverage of the rich physical interactions required for generalized world understanding. We introduce ACWM-Phys, a new benchmark for evaluating action-conditioned prediction under diverse physical dynamics in a clean, controllable simulation environment with a carefully designed action space. ACWM-Phys contains training and evaluation data spanning rigid-body dynamics, kinematics, deformable-object interactions, and particle dynamics. To evaluate both interpolation and generalization, we design in-distribution and out-of-distribution protocols with controlled shifts in interaction patterns or scene configurations. By building the benchmark in a fully controllable simulator, ACWM-Phys enables precise data collection, reproducible evaluation, and systematic analysis of model capabilities for physically grounded world modeling. Through systematic experiments on ACWM-DiT, we find that OoD generalization depends not only on the physical regime but also on effective task complexity: models generalize well on visually simple, low-dimensional interactions with clear geometric structure, but suffer larger drops on deformable contacts, high-dimensional control, and complex articulated motion. This suggests that the model still relies heavily on visual appearance patterns instead of fully learning the underlying physics. Ablations show that cross-attention improves high-dimensional action conditioning, causal VAEs outperform frame-wise encoders, and larger action spaces are harder to model but can improve generalization by providing richer control signals. These findings guide the design of physically grounded world models.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
\item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
\item[] Answer: \answerYes{}.
\item[] Justification: The abstract and introduction clearly state the benchmark, baseline model, evaluation protocol, and main empirical findings. The claims are limited to controlled simulation environments and supported by the reported experiments and ablations.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
\item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers.
\item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings.
\item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.
\end{itemize}

\item {\bf Limitations}
\item[] Question: Does the paper discuss the limitations of the work performed by the authors?
\item[] Answer: \answerYes{}.
\item[] Justification: The conclusion and case studies discuss limitations of current diffusion-based ACWMs, including OoD degradation, weak physical generalization, and failure cases in deformable, particle, and high-DoF settings. The paper also frames the benchmark as a diagnostic tool rather than claiming solved physical understanding.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper.
\item The authors are encouraged to create a separate ``Limitations'' section in their paper.
\item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
\item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
\item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
\item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
\item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
\item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
\end{itemize}

\item {\bf Theory assumptions and proofs}
\item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
\item[] Answer: \answerNA{}.
\item[] Justification: The paper is primarily empirical and benchmark-oriented, and does not introduce formal theoretical results requiring proofs. Mathematical formulations are provided to define the action-conditioned video diffusion objective.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that the paper does not include theoretical results.
\item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
\item All assumptions should be clearly stated or referenced in the statement of any theorems.
\item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition.
\item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
\item Theorems and Lemmas that the proof relies upon should be properly referenced.
\end{itemize}

\item {\bf Experimental result reproducibility}
\item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
\item[] Answer: \answerYes{}.
\item[] Justification: The paper describes the benchmark environments, InD/OoD protocols, action spaces, trajectory horizons, model design, training objective, evaluation metrics, and ablation settings. Dataset statistics and action-space definitions are further summarized in the appendix.
\item[] Guidelines:
\begin{itemize}
    \item The answer \answerNA{} means that the paper does not include experiments.
    \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
    \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
    \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
    \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
    \begin{enumerate}
        \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
        \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
        \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
        \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
    \end{enumerate}
\end{itemize}

\item {\bf Open access to data and code}
\item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
\item[] Answer: \answerYes{}.
\item[] Justification: We provide an anonymous link to view data and some video results; We will the code that after the paper is accepted.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that paper does not include experiments requiring code.
\item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}
) for more details.
\item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
\item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}
) for more details.
\item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
\item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
\item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
\item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
\end{itemize}

\item {\bf Experimental setting/details}
\item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
\item[] Answer: \answerYes{}.
\item[] Justification: The paper specifies the benchmark setup, InD/OoD splits, environment categories, action spaces, trajectory horizons, model variants, evaluation metrics, and ablation factors. Additional dataset and action-space details are provided in the appendix.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that the paper does not include experiments.
\item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
\item The full details can be provided either with the code, in appendix, or as supplemental material.
\end{itemize}

\item {\bf Experiment statistical significance}
\item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
\item[] Answer: \answerYes{}.
\item[] Justification: We follow the literature and use SSIM, MSE, PSNR metrics and faithfully report all the results during experiments.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that the paper does not include experiments.
\item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
\item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
\item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
\item The assumptions made should be given (e.g., Normally distributed errors).
\item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
\item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96% CI, if the hypothesis of Normality of errors is not verified.
\item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
\item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
\end{itemize}

\item {\bf Experiments compute resources}
\item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
\item[] Answer: \answerYes{}.
\item[] Justification: We put GPU type/ numbers and training steps in the experimental section.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that the paper does not include experiments.
\item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
\item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute.
\item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper).
\end{itemize}

\item {\bf Code of ethics}
\item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}
?
\item[] Answer: \answerYes{}.
\item[] Justification: The research uses controlled simulation environments and focuses on benchmarking action-conditioned video world models. We are not aware of any deviation from the NeurIPS Code of Ethics.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
\item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
\item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
\end{itemize}

\item {\bf Broader impacts}
\item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
\item[] Answer: \answerYes{}.
\item[] Justification: We put it in the front of the Appendix.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that there is no societal impact of the work performed.
\item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
\item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
\item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
\item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
\item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
\end{itemize}

\item {\bf Safeguards}
\item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
\item[] Answer: \answerNA{}.
\item[] Justification: The benchmark data are generated from controlled simulation environments and do not involve scraped human data, personal information, or high-risk pre-trained generative model release. Therefore, dedicated safeguards for high-risk data or model release are not applicable.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that the paper poses no such risks.
\item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters.
\item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
\item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
\end{itemize}

\item {\bf Licenses for existing assets}
\item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
\item[] Answer: \answerYes{}.
\item[] Justification: The paper cites existing models and methods used as foundations, including the pretrained video VAE, DiT, flow matching, and related ACWM and video diffusion works. We will ensure that the released code and documentation explicitly include license and terms-of-use information for all reused assets.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that the paper does not use existing assets.
\item The authors should cite the original paper that produced the code package or dataset.
\item The authors should state which version of the asset is used and, if possible, include a URL.
\item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
\item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
\item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
\item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
\item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
\end{itemize}

\item {\bf New assets}
\item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
\item[] Answer: \answerYes{}.
\item[] Justification: The paper introduces ACWM-Phys as a new benchmark and documents environment categories, dataset statistics, action spaces, trajectory horizons, and InD/OoD evaluation protocols. The project page, Hugging Face repository, and GitHub repository are intended to provide documentation alongside the released assets.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that the paper does not release new assets.
\item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc.
\item The paper should discuss whether and how consent was obtained from people whose asset is used.
\item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
\end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
\item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
\item[] Answer: \answerNA{}.
\item[] Justification: The paper does not involve crowdsourcing experiments or human-subject studies. All data are generated from controlled simulation environments.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
\item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper.
\item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector.
\end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
\item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
\item[] Answer: \answerNA{}.
\item[] Justification: The paper does not involve crowdsourcing, human-subject experiments, or collection of human data. Therefore, IRB approval or equivalent review is not applicable.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
\item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper.
\item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution.
\item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
\end{itemize}

\item {\bf Declaration of LLM usage}
\item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
\item[] Answer: \answerNo{}.
\item[] Justification: The core method, benchmark construction, experiments, and analysis do not use LLMs as an important, original, or non-standard research component. Any use of LLMs for writing, editing, or formatting does not affect the methodology, scientific rigor, or originality of the work.
\item[] Guidelines:
\begin{itemize}
\item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
\item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
\end{itemize}

\end{enumerate}

==> figures/vae_comparison_fig.tex <==
{\setlength{\tabcolsep}{1pt}%
\renewcommand{\arraystretch}{0.85}%
\scriptsize%
\begin{tabular}{@{}r@{\hspace{3pt}}>{\centering\arraybackslash}m{0.95\linewidth}@{}}
  \multicolumn{2}{@{}l@{}}{\textbf{Pour Water~---~Out-of-Distribution}} \\[1pt]
  \rotatebox{90}{\textbf{GT}}      & \includegraphics[width=\linewidth]{figures/vae_gt} \\[0.5pt]
  \rotatebox{90}{\textbf{WanVAE}}  & \includegraphics[width=\linewidth]{figures/vae_wan} \\[0.5pt]
  \rotatebox{90}{\textbf{FluxVAE}} & \includegraphics[width=\linewidth]{figures/vae_flux} \\
\end{tabular}}

==> tab_neurips/abl_actdim_table.tex <==
\begin{table}[h]
\centering
\caption{%
  \textbf{Action dimensionality ablation.}
  Cloth Move compares the reduced 3-DoF shared action against the full 8-DoF
  per-arm action space.
  Push Cube compares a single pusher ($d_a{=}2$) against two independent
  pushers ($d_a{=}4$).
}
\label{tab:abl_actdim}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{llc cccc}
\toprule
\textbf{Environment} & \textbf{Action Space} & $d_a$ &
  \multicolumn{2}{c}{\textbf{InD}} & \multicolumn{2}{c}{\textbf{OoD}} \\
\cmidrule(lr){4-5}\cmidrule(lr){6-7}
& & & MSE$\downarrow$ & PSNR$\uparrow$ & MSE$\downarrow$ & PSNR$\uparrow$ \\
\midrule
\multirow{2}{*}{Cloth Move}
  & Reduced (shared $\Delta xyz$) & 3 & 10.667 & 19.72 & 23.820 & 16.23 \\
  & Full (per-arm $\Delta$pose + grasp) & 8 & 12.861 & 18.91 & \phantom{0}6.922 & 21.60 \\
\midrule
\multirow{2}{*}{Push Cube}
  & Single pusher & 2 & 2.919 & 25.35 & 2.950 & 25.30 \\
  & Two pushers   & 4 & 6.034 & 22.19 & 9.997 & 20.00 \\
\bottomrule
\end{tabular}
\end{table}


==> tab_neurips/abl_action_cond_table.tex <==
\begin{table}[h]
\centering
\caption{%
  \textbf{Action conditioning ablation}: AdaLN vs.\ cross-attention across four environments
  spanning low and high action dimensionality.
  {\color{green!60!black}$\uparrow$}~better than AdaLN; {\color{red}$\downarrow$}~worse than AdaLN.
}
\label{tab:abl_action_cond}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l cccc cccc cccc cccc}
\toprule
&
\multicolumn{4}{c}{\textbf{Push Cube} ($d_a{=}2$)} &
\multicolumn{4}{c}{\textbf{Push Rope} ($d_a{=}2$)} &
\multicolumn{4}{c}{\textbf{Robot Arm} ($d_a{=}7$)} &
\multicolumn{4}{c}{\textbf{Cloth Move} ($d_a{=}8$)} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}\cmidrule(lr){14-17}
\textbf{Method} &
  \multicolumn{2}{c}{InD} & \multicolumn{2}{c}{OoD} &
  \multicolumn{2}{c}{InD} & \multicolumn{2}{c}{OoD} &
  \multicolumn{2}{c}{InD} & \multicolumn{2}{c}{OoD} &
  \multicolumn{2}{c}{InD} & \multicolumn{2}{c}{OoD} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\cmidrule(lr){10-11}\cmidrule(lr){12-13}
\cmidrule(lr){14-15}\cmidrule(lr){16-17}
& MSE & PSNR & MSE & PSNR
  & MSE & PSNR & MSE & PSNR
  & MSE & PSNR & MSE & PSNR
  & MSE & PSNR & MSE & PSNR \\
\midrule
AdaLN (ours)
  & 2.919 & 25.35 & 2.950 & 25.30
  & 0.214 & 36.70 & 0.329 & 34.83
  & 1.434 & 28.43 & 6.559 & 21.83
  & 10.667 & 19.72 & 23.820 & 16.23 \\
Cross-Attn
  & 3.105\worse & 25.08\worse & 3.033\worse & 25.18\worse
  & 0.216\worse & 36.65\worse & 0.334\worse & 34.77\worse
  & 0.691\better & 31.61\better & 4.596\better & 23.38\better
  & 12.405\worse & 19.06\worse & \phantom{0}5.220\better & 22.82\better \\
\bottomrule
\end{tabular}}
\end{table}


==> tab_neurips/abl_data_table.tex <==
\begin{table}[h]
\centering
\caption{%
  \textbf{Training data scaling ablation} on Push Cube and Pour Water.
  Models trained on 100\%, 50\%, and 25\% of available trajectories.
}
\label{tab:abl_data}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lc cccc cccc}
\toprule
& &
\multicolumn{4}{c}{\textbf{Push Cube}} &
\multicolumn{4}{c}{\textbf{Pour Water}} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
\textbf{Data} & \textbf{Trajs} &
  \multicolumn{2}{c}{InD} & \multicolumn{2}{c}{OoD} &
  \multicolumn{2}{c}{InD} & \multicolumn{2}{c}{OoD} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
& & MSE$\downarrow$ & PSNR$\uparrow$ & MSE$\downarrow$ & PSNR$\uparrow$
  & MSE$\downarrow$ & PSNR$\uparrow$ & MSE$\downarrow$ & PSNR$\uparrow$ \\
\midrule
100\% (full) & 1987 / 1000 & 2.919 & 25.35 & 2.950 & 25.30 & 2.630 & 25.80 & 3.488 & 24.57 \\
50\%         &  994 / 500  & 3.724 & 24.29 & 3.981 & 24.00 & 2.793 & 25.54 & 3.623 & 24.41 \\
25\%         &  497 / 250  & 5.318 & 22.74 & 5.891 & 22.30 & 3.882 & 24.11 & 4.689 & 23.29 \\
\bottomrule
\end{tabular}
\end{table}


==> tab_neurips/abl_scale_table.tex <==
\begin{table}[h]
\centering
\caption{%
  \textbf{Model scale ablation} on Cloth Move (3-DoF action, 50k steps) and Robot Arm (50k steps).
}
\label{tab:abl_scale}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lc cccc cccc}
\toprule
& &
\multicolumn{4}{c}{\textbf{Cloth Move}} &
\multicolumn{4}{c}{\textbf{Robot Arm}} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
\textbf{Model} & \textbf{Params} &
  \multicolumn{2}{c}{InD} & \multicolumn{2}{c}{OoD} &
  \multicolumn{2}{c}{InD} & \multicolumn{2}{c}{OoD} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
& & MSE$\downarrow$ & PSNR$\uparrow$ & MSE$\downarrow$ & PSNR$\uparrow$
  & MSE$\downarrow$ & PSNR$\uparrow$ & MSE$\downarrow$ & PSNR$\uparrow$ \\
\midrule
DiT-S & ${\approx}200$M & 10.776 & 19.68 & 22.416 & 16.49 & 1.452 & 28.38 & 6.552 & 21.84 \\
DiT-M & ${\approx}600$M & 10.248 & 19.89 & 20.031 & 16.98 & 1.247 & 29.04 & 4.891 & 23.11 \\
DiT-L & ${\approx}800$M &  9.985 & 20.01 & 18.876 & 17.24 & 1.183 & 29.27 & 4.453 & 23.51 \\
\bottomrule
\end{tabular}
\end{table}


==> tab_neurips/abl_vae_table.tex <==
\begin{table}[h]
\centering
\caption{%
  \textbf{Latent-space formulation ablation}: causal video VAE (Wan~2.1, $4\times$ temporal
  compression) vs.\ frame-independent image VAE (FLUX, $1\times$ temporal compression)
  on Pour Water.
}
\label{tab:abl_vae}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lc cccc}
\toprule
& &
\multicolumn{4}{c}{\textbf{Pour Water}} \\
\cmidrule(lr){3-6}
\textbf{VAE} & \textbf{Temp.\ Comp.} &
  \multicolumn{2}{c}{InD} & \multicolumn{2}{c}{OoD} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
& & MSE$\downarrow$ & PSNR$\uparrow$ & MSE$\downarrow$ & PSNR$\uparrow$ \\
\midrule
WanVAE (ours) & $4\times$ & 2.630 & 25.80 & 3.488 & 24.57 \\
FluxVAE       & $1\times$ & 3.241 & 24.89 & 3.895 & 24.09 \\
\bottomrule
\end{tabular}
\end{table}


==> tab_neurips/eval_table.tex <==
% General evaluation results: ACWM-DiT-S, steps=50, 100k training steps
\begin{table*}[t]
\centering
\label{tab:eval_main}
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{ll cccc cccc}
\toprule
& &
\multicolumn{4}{c}{\textbf{In-Distribution Test}} &
\multicolumn{4}{c}{\textbf{Out-of-Distribution Test}} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
\textbf{Category} & \textbf{Environment} &
  MSE$\downarrow$ & M-MSE$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ &
  MSE$\downarrow$ & M-MSE$\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ \\
\midrule
\multirow{2}{*}{Rigid}
  & Push Cube  & 2.919 & 10.513 & 0.955 & 25.35 & 2.950\worse  & \phantom{0}9.855        & 0.954\worse & 25.30\worse \\
  & Stack Cube & 5.516 & \phantom{0}9.550 & 0.889 & 22.58 & 6.996\worse  & 11.572\worse & 0.872\worse & 21.55\worse \\
\midrule
\multirow{2}{*}{Deformable}
  & Push Rope              & 0.214  & \phantom{0}0.805 & 0.988 & 36.70 & 0.329\worse  & \phantom{0}1.310\worse & 0.985\worse & 34.83\worse \\
  & Cloth Move$^{\dagger}$ & 10.667 & 40.331 & 0.920 & 19.72 & 23.820\worse & 69.678\worse & 0.864\worse & 16.23\worse \\
\midrule
\multirow{2}{*}{Particle}
  & Push Sand  & 0.519 & \phantom{0}2.343 & 0.975 & 32.85 & 1.526\worse & \phantom{0}6.830\worse & 0.941\worse & 28.16\worse \\
  & Pour Water & 2.630 & \phantom{0}8.092 & 0.911 & 25.80 & 3.488\worse & \phantom{0}9.714\worse & 0.874\worse & 24.57\worse \\
\midrule
\multirow{2}{*}{Kinematics}
  & Robot Arm & 1.434 & \phantom{0}5.769 & 0.969 & 28.43 & 6.559\worse & 23.614\worse & 0.902\worse & 21.83\worse \\
  & Reacher   & 0.260 & \phantom{0}1.349 & 0.992 & 35.85 & 0.272\worse & \phantom{0}1.407\worse & 0.992       & 35.65\worse \\
\bottomrule
\end{tabular}
\begin{tablenotes}
  \footnotesize
  \item[$\dagger$] Cloth Move involves large-scale deformation across most image pixels, yielding inherently higher MSE and lower PSNR than tasks with localised motion; values are not directly comparable across task types.                                                               
\end{tablenotes}
\end{threeparttable}
}
\caption{%
  \textbf{ACWM-DiT-S evaluation on ACWM-Phys} (diffusion steps\,=\,50, 100k training steps).
  MSE and Masked-MSE (M-MSE) are scaled by $10^{-3}$.
  PSNR is computed as $10\log_{10}(1/\text{MSE})$.
  {\color{red}$\downarrow$}~denotes OoD performance worse than InD.
}
\end{table*}


==> tabs/action_space_table.tex <==
% Action space summary table
\begin{table}[t]
\centering
\caption{%
  \textbf{Action space definitions across ACWM-Phys environments.}
  Actions are either \emph{absolute} target states or \emph{delta} (incremental) commands.
}
\label{tab:action_space}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{llcl}
\toprule
\textbf{Environment} & \textbf{Type} & \textbf{Dim} & \textbf{Semantics} \\
\midrule
Push Cube  & Absolute position  & 2 & Target $(x,y)$ pusher position on workspace \\
Stack Cube & Delta EE pose      & 7 & $(\Delta x,\Delta y,\Delta z,\Delta r_x,\Delta r_y,\Delta r_z)$ + gripper open/close \\
Push Rope  & Delta position     & 2 & 2D horizontal pole displacement $(\Delta x, \Delta z)$ \\
Cloth Move & Delta position      & 3 & $(\Delta x,\Delta y,\Delta z)$ dual-arm displacement$^*$ \\
Push Sand  & Delta board pose   & 7 & Board 3D position + 4D orientation delta \\
Pour Water & Delta cup pose     & 4 & $(\Delta x,\Delta y,\Delta z,\Delta\theta)$ cup tilt delta \\
Robot Arm  & Delta joint angles & 7 & Per-joint angle delta $\Delta\mathbf{q}\in\mathbb{R}^7$ \\
Reacher    & Joint torques      & 2 & Torques $(\tau_1,\tau_2)$ applied to two links \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/dataset_table.tex <==
% Dataset statistics table for ACWM-Phys
\begin{table}[t]
\centering
\caption{%
  \textbf{ACWM-Phys dataset statistics.}
  Each environment provides in-distribution (InD) and out-of-distribution (OoD) test splits
  with controlled distribution shifts. Action dim refers to the dimensionality of the
  action vector fed to ACWM-DiT; full action definitions are listed in Table~\ref{tab:action_space}.
}
\label{tab:dataset}
\small
\setlength{\tabcolsep}{5pt}
\begin{threeparttable}
\begin{tabular}{llccccc}
\toprule
\textbf{Category} & \textbf{Environment} & \textbf{Train} & \textbf{InD Test} & \textbf{OoD Test} & \textbf{Act.\ Dim} & \textbf{Horizon} \\
\midrule
\multirow{2}{*}{Rigid Dynamics}
  & Push Cube   & 1,987 & 100 & 100 & 2 & $\sim$66 \\
  & Stack Cube  & 1,987 & 100 & 100 & 7 & $\sim$57 \\
\midrule
\multirow{2}{*}{Deformable}
  & Push Rope       & 1,987 & 100 & 100 & 2 & 64 \\
  & Cloth Move$^*$  & 1,987 & 100 & 100 & 3 & 64 \\
\midrule
\multirow{2}{*}{Particle}
  & Push Sand   & 1,784 & 100 & 100 & 7 & 64 \\
  & Pour Water  & 1,000 &  50 &  50 & 4 & 300 \\
\midrule
\multirow{2}{*}{Kinematics}
  & Robot Arm   & 1,987 & 100 & 100 & 7 & 64 \\
  & Reacher     & 1,987 & 100 & 100 & 2 & 50  \\
\midrule
\textbf{Total}    & 8 environments       & \textbf{14,706} & \textbf{750} & \textbf{750} & 2--7 & 50--300 \\
\bottomrule
\multicolumn{7}{l}{\footnotesize $^*$Cloth Move uses reduced 3-dim actions; 8-dim variant used in action-dimension ablation.}
\end{tabular}
\end{threeparttable}
\end{table}


==> tabs/relatedworks.tex <==
% in preamble
% \usepackage{booktabs}
% \usepackage{threeparttable}
% \usepackage{pifont}
% \newcommand{\cmark}{\ding{51}}
% \newcommand{\xmark}{\ding{55}}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.3}
\begin{threeparttable}
\resizebox{\textwidth}{!}{
\begin{tabular}{l l c c c c}
\toprule
\textbf{Benchmark} & \textbf{Type} & \textbf{Action-conditioned} & \textbf{Rich Physics} & \textbf{Data Scale} & \textbf{ID+OOD} \\
\midrule
Solaris~\cite{savva2026solaris}
& Multi-Player Minecraft
& \cmark
& \xmark
& 9k videos
& \xmark \\

Dreamer4~\cite{dreamer4}
& Minecraft
& \cmark
& \xmark
& 2.5K hour gameplay
& \xmark \\

DROID~\cite{khazatsky2024droid}
& Expert manipulation
& \cmark
& \xmark
& 76K trajectories
& \xmark \\

RECON~\cite{recondataset}
& Egocentric navigation
& \cmark
& \xmark
& 5K trajectories
& \xmark \\

Physics-IQ~\cite{motamed2026generative}
& Passive physics evaluation
& \xmark
& \cmark
& 396 videos
& \xmark \\

WISA~\cite{wang2025wisa}
& Passive physics evaluation
& \xmark
& \cmark
& 32K videos
& \xmark \\

PhysInOne~\cite{physinone}
& Synthetic physics interaction
& \xmark
& \cmark
& 2M videos
& \xmark \\

\midrule
\textbf{ACWM-Phys (ours)}
& \textbf{Synthetic physics interaction}
& \textbf{\cmark}
& \textbf{\cmark}
& \textbf{15k videos}
& \textbf{\cmark} \\
\bottomrule
\end{tabular}
}
\end{threeparttable}
\caption{\textbf{Comparison of ACWM-Phys with existing action-conditioned and physics-related benchmarks.} Benchmarks used for training action-conditioned world models generally lack rich and diverse physical interactions, whereas existing physics-focused benchmarks are typically not action-conditioned. Also, most prior benchmarks do not include both in-distribution and out-of-distribution evaluations}
\label{tab:benchmark_comparison}
\end{table*}

==> tex/dataset_and_model.tex <==
\section{Investigating ACWMs for Learning Generalized Physical Interactions}

%% ─────────────────────────────────────────────────────────────────────────────
\subsection{ACWM-Phys: A Benchmark Suite for Rich Physical Interactions}

ACWM-Phys comprises eight robotic simulation environments grouped into four categories
of physical interaction: rigid-body dynamics, deformable-object dynamics, particle dynamics,
and kinematics (Figure~\ref{fig:dataset_overview}).  Each environment provides separate
in-distribution (InD) training and test splits, as well as an out-of-distribution (OoD)
test split with a controlled distribution shift.  Dataset sizes and action specifications
are provided in Appendix~\ref{app:dataset_stats}.

\input{figures/dataset_overview_fig}

\subsubsection{Categories of Physical Interactions}

\textbf{Rigid-Body Dynamics.}
\texttt{Push Cube} places a circular pusher on a large flat workspace and tasks the agent
with moving one to five colored cubes.  The action $\mathbf{a}\in\mathbb{R}^{2}$ specifies
the \emph{absolute} 2D target position of the pusher on the workspace, and the pusher is
driven there by a PD controller.
\texttt{Stack Cube} uses a Franka Panda manipulator that must pick up a red cube and
place it on top of a green one.  The action $\mathbf{a}\in\mathbb{R}^{7}$ is a \emph{delta}
six-DoF end-effector pose together with a scalar gripper open/close command.

\textbf{Deformable-Object Dynamics.}
\texttt{Push Rope} simulates a flexible rope on a tabletop ((PyFlex~\cite{li2018learning})) and
moves it with a pole pusher.  The action $\mathbf{a}=(\Delta x,\Delta z)\in\mathbb{R}^{2}$
is a 2D horizontal displacement delta of the pole.
\texttt{Cloth Move} uses a dual-arm system that pushes a deformable cloth over a fixed
sphere obstacle.  The action $\mathbf{a}\in\mathbb{R}^{3}$ is a shared 3D position
delta $(\Delta x,\Delta y,\Delta z)$ applied to the dual-arm end-effectors.
We use this reduced action space in the main benchmark; the full 8-dim variant
(per-arm delta + grasp) is studied in the action-dimension ablation (Section~\ref{sec:experiments}).

\textbf{Particle Dynamics.}
\texttt{Push Sand} features a flat board pusher that rearranges a pile of granular
material (PyFleX).  The action $\mathbf{a}\in\mathbb{R}^{7}$ encodes the full
three-dimensional position and orientation delta of the board.
\texttt{Pour Water} tilts a cup to pour fluid into a stationary container (PyFlex).
The action $\mathbf{a}=(\Delta x,\Delta y,\Delta z,\Delta\theta)\in\mathbb{R}^{4}$
represents incremental deltas of the cup's Cartesian position and tilt angle,
produced by a three-phase spring-damper pour controller.

\textbf{Kinematics.}
\texttt{Robot Arm} tasks a 7-DoF Franka Panda with reaching randomized end-effector
goals, simulated in Isaac Sim with cuRobo motion planning.  The action
$\mathbf{a}=\Delta\mathbf{q}\in\mathbb{R}^{7}$ is a vector of per-joint angle deltas.
\texttt{Reacher} controls a two-link planar arm in a 2D horizontal plane (MuJoCo~\cite{todorov2012mujoco}) to reach
goal positions.  The action $\mathbf{a}=(\tau_1,\tau_2)\in\mathbb{R}^{2}$ directly
specifies joint torques applied to the two links.


\subsubsection{In-Distribution and Out-of-Distribution Evaluation Protocols}

A central design principle of ACWM-Phys is that \emph{every} environment supports
a controlled, physically motivated distribution shift between the InD and OoD splits.
Rather than applying random perturbations, we shift the physical parameters or
workspace regions that most directly challenge the generalization of a learned world model:

\begin{itemize}[leftmargin=1.4em, itemsep=1pt]
  \item \textbf{Rigid}: Push Cube has only 3 cubes for training, but use 1 or 4+ cubes for testing; Stack Cube
        perturbs the target placement in one of four directions (up/down/left/right).
  \item \textbf{Deformable}: Push Rope use shorter of longer rope during testing; Cloth Move
        changes square-cloth size (InD: 100--150 particles/side; OoD smaller: 50--100,
        OoD larger: 150--200).
  \item \textbf{Particle}: Push Sand doubles the particle count from InD (50k--72k)
        to OoD (144k); Pour Water shifts the water level from InD values
        (20, 24, 32 layers) to OoD values (14 or 48 layers).
  \item \textbf{Kinematics}: Robot Arm expands the goal workspace(a cubic area) by $\pm 0.1$\,m
        beyond training bounds; Reacher restricts OoD goals to $20^\circ$ corner
        sectors ($45^\circ/135^\circ/225^\circ/315^\circ$) excluded from training.
\end{itemize}

Because all environments are fully simulated, the OoD parameters are exactly reproducible
and free from sensor noise, enabling precise measurement of the generalization gap.
This contrasts with real-robot benchmarks~\cite{khazatsky2024droid}, where distribution
shift is difficult to quantify or control.  Evaluation follows a shared protocol: models
are trained solely on InD data and evaluated on both InD test and OoD test trajectories. Regarding evaluation metrics, we use MSE and SSIM~\cite{psnr} as classical pixel-level measures of reconstruction quality; PSNR to quantify the signal-to-noise ratio; we also introduce Masked-MSE (M-MSE) to focus on the motion-relevant region, computed by restricting the MSE to pixels whose ground-truth intensity changes by
   more than a threshold across consecutive frames, thereby down-weighting the static background and emphasizing prediction accuracy where physical dynamics actually occur.
%% ─────────────────────────────────────────────────────────────────────────────
\subsection{ACWM-DiT: An Action-Conditioned Video Diffusion Transformer in Latent Space}




\begin{figure}[t]
  \centering
  \begin{minipage}[c]{0.53\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/model.pdf}
  \end{minipage}
  \hspace{0.02\linewidth}
  \begin{minipage}[c]{0.40\linewidth}
    \caption{%
      \textbf{ACWM-DiT architecture.}
      Noisy latent tokens $\mathbf{z}_{1:T_l}$ (conditioning frames at $\sigma{=}0$,
      predicted frames at diffusion step $\sigma$) are processed by $N$ stacked DiT blocks
      with alternating spatial and temporal self-attention, modulated via AdaLN from a
      joint conditioning signal $\mathbf{c}=\mathbf{e}_t+\hat{\mathbf{a}}$ formed by
      summing the timestep embedding and the temporally compressed action embedding.
    }
    \label{fig:model_arch}
  \end{minipage}
\end{figure}

\paragraph{Overall Architecture}

ACWM-DiT (Figure~\ref{fig:model_arch}) is a latent video diffusion transformer trained
with flow matching to predict future observation trajectories conditioned on past
observations and a sequence of actions.

\textbf{Video VAE.}
Following Wan~2.1~\cite{wan2025wan}, we use a pretrained causal VAE that compresses a
video $\mathbf{o}_{1:T}\in\mathbb{R}^{T\times 3\times H\times W}$ into latent tokens
$\mathbf{z}\in\mathbb{R}^{T_l\times\frac{H}{8}\times\frac{W}{8}\times 16}$, applying
$8\times$ spatial compression, $4\times$ temporal compression, and a 16-channel latent
space.  All VAE weights are frozen throughout training.

\textbf{Video DiT Backbone.}
The denoiser is a bidirectional (non-causal) transformer that operates on
spatiotemporally patchified latents (spatial patch size~2).  Each of the $N$ transformer
blocks consists of a spatial self-attention layer (attending over the
$\frac{H}{16}\times\frac{W}{16}$ spatial patches within each frame) followed by a
temporal self-attention layer attending across $T_l$ latent timesteps at each spatial
location.  Rotary Position Embeddings (RoPE) are used in both layers.
Observation-conditioning frames are passed at noise level $\sigma{=}0$ while predicted
frames are noised at the current diffusion step $\sigma$; this allows the model to
attend bidirectionally over both clean context and noisy future tokens.
Conditioning on the diffusion timestep and actions is applied through Adaptive Layer
Normalization (AdaLN), which uses the joint signal $\mathbf{c}$ to produce per-step
scale and shift parameters $(\gamma,\beta,\alpha)$ at every block.
We study two model scales: \textbf{DiT-S} (hidden dim~768, 10~layers, 12~heads,
${\approx}200$M parameters) and \textbf{DiT-M} (hidden dim~1024, 16~layers, 16~heads,
${\approx}600$M parameters).

\textbf{Flow Matching.}
Training follows the latent-space flow matching objective defined in
Section~\ref{sec:background} with a linear interpolation path and shift
parameter~$s{=}5.0$.  Training losses are weighted by a Gaussian envelope centered at
diffusion step~500 to focus supervision on intermediate noise levels.  We use 1000
training steps and 50 inference denoising steps.

\paragraph{Action Conditioning Module}

Actions are integrated via a dedicated \emph{ActionEmbedder} module that maps the
pixel-rate action sequence to the latent temporal resolution in two stages.
First, an MLP (Linear$\to$SiLU$\to$Linear) projects each action vector from its
environment-specific dimension $d_a$ to the DiT hidden dimension~$d$.
Second, a 1D strided convolution (kernel size~3, stride~$r{=}4$, matching the
VAE's $4\times$ temporal compression factor) downsamples the sequence from
$1 + r(T_l{-}1)$ pixel-rate steps to $T_l$ latent-rate tokens, producing
$\hat{\mathbf{a}}\in\mathbb{R}^{T_l\times d}$.

The action embedding is summed with the per-step timestep embedding to form the
joint conditioning signal
$\mathbf{c} = \mathbf{c}_t + \hat{\mathbf{a}} \;\in\; \mathbb{R}^{T_l\times d},$
which is then broadcast into every DiT block via AdaLN, modulating the scale and
shift applied after each layer normalization.
This design couples action information with the diffusion timestep and propagates it
uniformly across all spatial and temporal attention operations without requiring
additional cross-attention layers or token-sequence modifications.
For the standard training setting we use no action dropout ($p_{\text{drop}}{=}0$);
ablations on classifier-free guidance are left to future work.


==> tex/experiments.tex <==

\section{Experiments}
\label{sec:experiments}

%% ─────────────────────────────────────────────────────────────────────────────
\paragraph{Training Setup} All models are trained seperately from scratch with the AdamW optimizer at a learning rate of $10^{-4}$
with gradient clipping at 1.0.
We train for 100k steps with a batch size of 4 on 8 H100 GPUs for each task.
The flow-matching scheduler uses 1000 noise levels with a shift parameter $s{=}5.0$
and a Gaussian weighting envelope centered at noise step 500 to focus supervision
on intermediate denoising levels.
Video observations are encoded by the frozen Wan~2.1 causal VAE into latent tokens of
spatial resolution $H/8{\times}W/8$ with 16 channels and $4\times$ temporal compression.
Input sequences are padded/trimmed to a fixed latent length of $T_l{=}37$ tokens.
All environments are resized to $240{\times}240$ pixels prior to encoding,
except Push Sand which uses $240{\times}400$ to preserve its landscape aspect ratio.
All environments are trained with the AdaLN action-conditioning variant; cross-attention conditioning is evaluated separately in the ablation studies (Section \ref{sec:experiments}).

%% ─────────────────────────────────────────────────────────────────────────────
\subsection{Main Results}

Table~\ref{tab:eval_main} reports ACWM-DiT-S on all eight ACWM-Phys environments
at 100k training steps and 50 inference steps. 
\input{tabs/eval_table}

\paragraph{InD performance.}
ACWM-DiT-S achieves strong in-distribution performance across all four physics categories. Environments with simpler, repetitive dynamics achieve the highest fidelity: Push Rope (M-MSE 2.61, SSIM 0.988) and Reacher (M-MSE 5.63, SSIM 0.992) are predicted with near-perfect structural similarity and low motion-region error, indicating that the model captures both dynamic foreground behavior and global spatial coherence. Stack Cube (M-MSE 10.93, SSIM 0.889) and Cloth Move (M-MSE 63.68, SSIM 0.920) pose the greatest challenge: the lower InD SSIM for Stack Cube is mainly due to large foreground motion of the robot arm, which introduces substantial dynamic changes across frames, while Cloth Move's substantially higher M-MSE shows that large-scale deformation leads to much larger errors in physically dynamic regions even within the training distribution. 

\paragraph{OoD generalization.}
A consistent degradation is observed under distribution shift, especially in motion-sensitive regions. The largest OoD increases in M-MSE occur for Robot Arm ($\Delta$M-MSE $= +40.35$, $\Delta$SSIM $= -0.067$) and Cloth Move ($\Delta$M-MSE $= +29.99$, $\Delta$SSIM $= -0.056$), suggesting that the model struggles to extrapolate to unseen configurations involving large articulated motion or large-scale deformation. This indicates that ACWM-DiT-S still relies partly on training-distribution regularities rather than fully internalizing general physical dynamics.
Notably, OoD robustness correlates more strongly with task complexity than with physics category. Push Cube ($\Delta$SSIM $= -0.001$) and Reacher ($\Delta$SSIM $= 0.000$) maintain nearly identical structural similarity across distributions, as their dynamics are governed by relatively low-dimensional geometric constraints that transfer well across workspace configurations. Push Sand shows a clear increase in motion-region error ($\Delta$M-MSE $= +9.32$) while retaining moderate structural similarity (OoD SSIM $=0.941$, $\Delta$SSIM $= -0.034$), suggesting that the model preserves coarse granular appearance but struggles to accurately predict fine-grained particle redistribution under larger distribution shifts. Pour Water is comparatively more robust in M-MSE ($\Delta$M-MSE $= +2.40$), although its SSIM still decreases ($\Delta$SSIM $= -0.037$), likely because the repeatable pouring trajectory constrains the overall structure even under unseen water volumes.

\paragraph{Generalization summary.}
Across environments, generalization ability is governed primarily by the dimensionality
of the underlying state space rather than by physics category:
environments whose dynamics reduce to low-dimensional geometric rules
(rigid-body translation, joint-angle trajectories) transfer robustly to unseen configurations,
while high-dimensional or stochastic dynamics (cloth deformation, granular flow)
expose the model's reliance on appearance statistics over learned physical structure.

\begin{figure}[h]
  \centering
  \input{figures/case_pour_water_fig}
  \caption{%
    \textbf{Case study: Pour Water.}
    GT (top) and predicted (bottom) frames at four evenly-spaced timesteps.
    Two InD episodes (top block) and two OoD episodes (bottom block) with less water (left) and more water (right);
    The model generalises well for InD but shows water amount change in OoD.
  }
  \label{fig:case_pour_water}
\end{figure}

\begin{figure}[h]
  \centering
  \input{figures/case_push_cube_fig}
  \caption{%
    \textbf{Case study: Push Cube.}
    GT (top) and predicted (bottom) frames at four evenly-spaced timesteps.
    Two InD episodes (top block) and two OoD episodes (bottom block) show
    diverse cube configurations, with one cube  (left) and four cubes (right).
    The model accurately tracks cube positions and push trajectories
    across both distributions.
  }
  \label{fig:case_push_cube}
\end{figure}
\paragraph{Case study: Pour Water.}

The model correctly predicts the pouring trajectory and the general fluid dynamics
for in-distribution water levels (Figure~\ref{fig:case_pour_water} in Appendix).
Under OoD shifts (fewer or far more water layers than seen during training), the model
tends to generate visually plausible but physically incorrect fill levels,
highlighting the gap between perceptual quality and true physical understanding.

\paragraph{Case study: Push Cubes.}
Figure~\ref{fig:case_push_cube} contrasts two OoD regimes: a single cube pushed to
an out-of-distribution workspace position, and a scene with 4+ cubes (unseen during training).
The model accurately tracks rigid-body trajectories in both cases,
including contact events and post-push resting positions.
The low OoD degradation reflects that the
underlying pushing dynamics are governed by low-dimensional geometric constraints
that generalise across both workspace regions and object counts unseen during training.





More per-environment case studies for all remaining environments are provided
in Appendix~\ref{app:case_studies}.






%% ─────────────────────────────────────────────────────────────────────────────
\subsection{Ablation Studies}

\definecolor{lskyblue}{RGB}{135,206,250}
\newcommand{\finding}[1]{%
  \begin{tcolorbox}[
    colback=lskyblue!22!white,
    colframe=lskyblue!55!white,
    boxrule=0.5pt, arc=4pt,
    left=7pt, right=7pt, top=4pt, bottom=4pt,
    before skip=4pt, after skip=6pt,
  ]
  \small #1
  \end{tcolorbox}%
}

We conduct ablation studies along the following axes to provide further insights:
model scale, action-conditioning mechanism, latent-space formulation,
training data volume, and action dimensionality.

%% ── 1. Model Scale ────────────────────────────────────────────────────────────
\finding{\textbf{Model Scale.} Scaling model capacity consistently improves OoD robustness more than InD accuracy,
suggesting larger models better internalize physical structure rather than memorizing appearance statistics.
Gains diminish from DiT-M to DiT-L at the current data scale.}
Table~\ref{tab:abl_scale} compares
DiT-S (${\approx}200$M), DiT-M (${\approx}600$M), and DiT-L (${\approx}800$M)
on Cloth Move (deformable) and Robot Arm (kinematics),
two environments that represent qualitatively different physical interaction regimes.
Scaling from DiT-S to DiT-M consistently improves both InD and OoD performance,
with larger gains on OoD, suggesting that model capacity helps internalize physical
structure rather than merely memorizing training appearances.
Gains from DiT-M to DiT-L are more modest, indicating diminishing returns at this data scale.

\input{tabs/abl_scale_table}

%% ── 2. Action Conditioning ────────────────────────────────────────────────────
\finding{\textbf{Action Conditioning.} Cross-attention is mainly beneficial for high-dimensional action spaces. For low-dimensional controls ($d_a{=}2$), AdaLN performs similarly or slightly better, while cross-attention gives clear gains on Robot Arm and modest OoD gains on Cloth Move.}

We compare AdaLN-based action conditioning with a cross-attention variant that injects action tokens through dedicated cross-attention layers. As shown in Table~\ref{tab:abl_action_cond}, cross-attention brings no benefit on Push Cube and Push Rope ($d_a{=}2$), where AdaLN already captures simple displacement controls effectively. In contrast, for Robot Arm ($d_a{=}7$), cross-attention substantially improves both InD and OoD performance, suggesting better binding between joint commands and articulated motion. For Cloth Move ($d_a{=}8$), cross-attention slightly hurts InD performance but modestly improves OoD performance. Overall, cross-attention is most useful when actions are high-dimensional and require structured spatial-temporal grounding.

\input{tabs/abl_action_cond_table}

%% ── 3. Latent-Space Formulation ───────────────────────────────────────────────
\finding{\textbf{Latent-Space Choice.} A temporally-aware causal VAE outperforms frame-independent VAE}
The Wan~2.1 causal VAE~\cite{wan21github} applies $4\times$ temporal compression, coupling consecutive frames
in the latent space.
We ablate this against a frame-independent image VAE (FLUX VAE~\cite{flux2024}),
which encodes each frame independently ($1\times$ temporal compression).
Table~\ref{tab:abl_vae} reports results on Pour Water, a particle-dynamics environment
where per-frame spatial detail matters.
WanVAE outperforms FluxVAE on both InD (25.80\,dB vs.\ 24.89\,dB) and OoD
(24.57\,dB vs.\ 24.09\,dB), indicating that temporally-aware latent representations
are beneficial even for highly stochastic particle dynamics.

\input{tabs/abl_vae_table}

%% ── 4. Training Data Scaling ──────────────────────────────────────────────────
\finding{\textbf{Data Efficiency.} Data efficiency is governed by geometric variability: Pour Water degrades
gracefully with less data due to its single repeatable pouring motion, while
Push Cube degrades sharply as it requires diverse trajectory coverage over a wide workspace.}
We train DiT-S on Push Cube and Pour Water using 100\%, 50\%, and 25\% of the
available training trajectories (Table~\ref{tab:abl_data}).
Both environments show  degradation as data is reduced.
Push Cube degrades sharply,
indicating that diverse cube configurations and push directions require broad
trajectory coverage to generalize.
Pour Water is substantially more data-efficient: at 50\% data the InD drop is
only $0.26$\,dB, and even at 25\% it retains reasonable performance ($-1.69$\,dB),
likely because its dynamics are governed by a single repeatable pouring motion
with limited geometric variability.

\input{tabs/abl_data_table}

%% ── 5. Action Dimensionality ──────────────────────────────────────────────────
\finding{\textbf{Action Dimensionality.} Higher-dimensional actions make prediction harder, but can improve OoD generalization when they provide more informative control signals and richer observation.}
Table~\ref{tab:abl_actdim} compares action-space variants for Cloth Move and Push Cube. For Cloth Move, we use the full action space by allowing the two grippers to move independently, providing more detailed control over the deformable object. This substantially improves OoD MSE, suggesting that richer action signals help the model infer two-arm cloth dynamics. In contrast, for Push Cube, adding a second pusher increases interaction complexity without providing the same informative benefit, resulting in higher MSE in both InD and OoD settings.


==> tex/experiments_neurips.tex <==

\section{Experiments}
\label{sec:experiments}

%% ─────────────────────────────────────────────────────────────────────────────
\subsection{Training Setup}

All models are trained with the AdamW optimizer at a learning rate of $10^{-4}$
with gradient clipping at 1.0.
We train for 100k steps with a batch size of 4 on 8 H100 GPUs for each task.
The flow-matching scheduler uses 1000 noise levels with a shift parameter $s{=}5.0$
and a Gaussian weighting envelope centered at noise step 500 to focus supervision
on intermediate denoising levels.
Video observations are encoded by the frozen Wan~2.1 causal VAE into latent tokens of
spatial resolution $H/8{\times}W/8$ with 16 channels and $4\times$ temporal compression.
Input sequences are padded/trimmed to a fixed latent length of $T_l{=}37$ tokens.
All environments are resized to $240{\times}240$ pixels prior to encoding,
except Push Sand which uses $240{\times}400$ to preserve its landscape aspect ratio.
All environments are trained with the AdaLN action-conditioning variant; cross-attention conditioning is evaluated separately in the ablation studies (Section \ref{sec:experiments}).

%% ─────────────────────────────────────────────────────────────────────────────
\subsection{Main Results}

Table~\ref{tab:eval_main} reports ACWM-DiT-S on all eight ACWM-Phys environments
at 100k training steps and 50 inference steps. We put influence of sampling steps in the Appendix~\ref{app:steps_curves}.

\input{tabs/eval_table}

\paragraph{InD performance.}
ACWM-DiT-S achieves strong in-distribution performance across all four physics categories.
Environments with simpler, repetitive dynamics achieve the highest fidelity:
Push Rope (PSNR 36.70, SSIM 0.988) and Reacher (PSNR 35.85, SSIM 0.992) are predicted
with near-perfect structural similarity, indicating the model captures both pixel-level
accuracy and global spatial coherence.
Stack Cube (PSNR 22.58, SSIM 0.889) and Cloth Move (PSNR 19.72, SSIM 0.920) pose the
greatest challenge: the lower InD SSIM for Stack Cube reflects its contact-rich
multi-object interactions that produce complex, hard-to-reconstruct configurations,
while Cloth Move's large-scale deformation degrades both pixel accuracy and structural
coherence even within the training distribution.

\paragraph{OoD generalization.}
A consistent drop in both PSNR and SSIM is observed under distribution shift.
The degradation is most severe for Robot Arm ($\Delta$PSNR $= -6.60$\,dB,
$\Delta$SSIM $= -0.067$) and Cloth Move ($\Delta$PSNR $= -3.49$\,dB,
$\Delta$SSIM $= -0.056$), confirming that the model relies on appearance statistics
rather than internalizing physical laws.
Notably, OoD robustness correlates more strongly with task complexity than with physics
category: Push Cube ($\Delta$SSIM $= -0.001$) and Reacher ($\Delta$SSIM $= 0.000$)
maintain near-identical structural similarity across distributions, as their dynamics
are governed by low-dimensional geometric constraints that transfer across workspace
configurations.
Push Sand shows a sharp PSNR drop ($-4.69$\,dB) but retains moderate SSIM
(OoD 0.941, $\Delta$SSIM $= -0.034$), suggesting the model preserves coarse granular
texture but fails to correctly predict particle count under large distribution shifts.
Pour Water is more robust in both metrics ($\Delta$PSNR $= -1.23$\,dB,
$\Delta$SSIM $= -0.037$), as the repeatable pouring trajectory constrains structural
variability even at unseen water volumes.

\paragraph{Generalization summary.}
Across environments, generalization ability is governed primarily by the dimensionality
of the underlying state space rather than by physics category:
environments whose dynamics reduce to low-dimensional geometric rules
(rigid-body translation, joint-angle trajectories) transfer robustly to unseen configurations,
while high-dimensional or stochastic dynamics (cloth deformation, granular flow)
expose the model's reliance on appearance statistics over learned physical structure.

\paragraph{Case study: Pour Water.}
Pour Water exhibits a particularly instructive pattern.
The model correctly predicts the pouring trajectory and the general fluid dynamics
for in-distribution water levels.
Under OoD shifts (fewer or far more water layers than seen during training), the model
tends to generate visually plausible but physically incorrect fill levels,
highlighting the gap between perceptual quality and true physical understanding.

\paragraph{Case study: Push Cubes.}
Figure~\ref{fig:case_push_cube} contrasts two OoD regimes: a single cube pushed to
an out-of-distribution workspace position, and a scene with 4+ cubes (unseen during training).
The model accurately tracks rigid-body trajectories in both cases,
including contact events and post-push resting positions.
The low OoD degradation ($\Delta$PSNR $= -0.05$\,dB) reflects that the
underlying pushing dynamics are governed by low-dimensional geometric constraints
that generalise across both workspace regions and object counts unseen during training.
Additional per-environment case studies for all remaining environments are provided
in Appendix~\ref{app:case_studies}.

\begin{figure}[h]
  \centering
  \input{figures/case_pour_water_fig}
  \caption{%
    \textbf{Case study: Pour Water.}
    GT (top) and predicted (bottom) frames at four evenly-spaced timesteps.
    Two InD episodes (top block) and two OoD episodes (bottom block) contrast
    low and high water-quantity regimes.
    The model generalises well in-distribution but shows fill-level errors
    under OoD water quantities.
  }
  \label{fig:case_pour_water}
\end{figure}

\begin{figure}[h]
  \centering
  \input{figures/case_push_cube_fig}
  \caption{%
    \textbf{Case study: Push Cube.}
    GT (top) and predicted (bottom) frames at four evenly-spaced timesteps.
    Two InD episodes (top block) and two OoD episodes (bottom block) show
    diverse cube configurations.
    The model accurately tracks cube positions and push trajectories
    across both distributions.
  }
  \label{fig:case_push_cube}
\end{figure}

\begin{figure}[h]
  \centering
  \input{figures/ar_generation_fig}
  \caption{%
    \textbf{Auto-regressive Generation.}
    The model generates frames $1{\to}37$ (blue) conditioned on the first frame,
    then generates frames $37{\to}T$ (red) conditioned on the last predicted frame
    of the first window.
    GT (top) and predicted (bottom) frames at four evenly-spaced timesteps per window.
  }
  \label{fig:ar_generation}
\end{figure}

%% ─────────────────────────────────────────────────────────────────────────────
\subsection{Ablation Studies}

\definecolor{lskyblue}{RGB}{135,206,250}
\newcommand{\finding}[1]{%
  \begin{tcolorbox}[
    colback=lskyblue!22!white,
    colframe=lskyblue!55!white,
    boxrule=0.5pt, arc=4pt,
    left=7pt, right=7pt, top=4pt, bottom=4pt,
    before skip=4pt, after skip=6pt,
  ]
  \small #1
  \end{tcolorbox}%
}

We conduct ablation studies on five design axes:
model scale, action-conditioning mechanism, latent-space formulation,
training data volume, and action dimensionality.
Unless otherwise noted, ablations are evaluated at 50k training steps with 50 inference steps.
MSE values are scaled by $10^{-3}$.

%% ── 1. Model Scale ────────────────────────────────────────────────────────────
\finding{\textbf{Model Scale.} Scaling model capacity consistently improves OoD robustness more than InD accuracy,
suggesting larger models better internalize physical structure rather than memorizing appearance statistics.
Gains diminish from DiT-M to DiT-L at the current data scale.}
Table~\ref{tab:abl_scale} compares
DiT-S (${\approx}200$M), DiT-M (${\approx}600$M), and DiT-L (${\approx}800$M)
on Cloth Move (deformable) and Robot Arm (kinematics),
two environments that represent qualitatively different physical interaction regimes.
Scaling from DiT-S to DiT-M consistently improves both InD and OoD performance,
with larger gains on OoD, suggesting that model capacity helps internalize physical
structure rather than merely memorizing training appearances.
Gains from DiT-M to DiT-L are more modest, indicating diminishing returns at this data scale.

\input{tabs/abl_scale_table}

%% ── 2. Action Conditioning ────────────────────────────────────────────────────
\finding{\textbf{Action Conditioning.} Cross-attention outperforms AdaLN only when action dimensionality is high.
At $d_a{=}2$, both methods perform similarly; at $d_a{=}8$, cross-attention yields
large OoD gains (especially for cloth-move), as AdaLN's global scale-shift becomes
a bottleneck for complex per-arm control signals.}
We compare the default AdaLN-based action conditioning against a cross-attention
alternative, where action tokens are injected via dedicated cross-attention layers
interleaved between spatial and temporal self-attention.
Table~\ref{tab:abl_action_cond} reports results across four environments spanning
low and high action dimensionality: Push Cube ($d_a{=}2$, rigid), Push Rope
($d_a{=}2$, deformable), Robot Arm ($d_a{=}7$, kinematics), and Cloth Move
($d_a{=}8$, deformable).
The benefit of cross-attention scales clearly with action dimensionality and
task structure rather than physics category.
At $d_a{=}2$, cross-attention yields no gain for either Push Cube
(OoD $25.30\,\to\,25.18$\,dB) or Push Rope (OoD $34.83\,\to\,34.77$\,dB):
low-dimensional displacements are trivially captured by AdaLN's global
scale-shift, making explicit token-level binding redundant.
Gains become substantial for Robot Arm ($d_a{=}7$), where cross-attention
recovers a large InD improvement ($28.43\,\to\,31.61$\,dB, $+3.18$\,dB)
by tightly coupling each joint-angle command to its corresponding latent frame.
The effect is most dramatic for Cloth Move ($d_a{=}8$), where OoD performance
jumps from $16.23$ to $22.82$\,dB ($+6.59$\,dB):
with eight per-arm degrees of freedom, AdaLN's single conditioning vector
becomes a severe bottleneck, while cross-attention's per-timestep injection is
critical for generalizing to unseen cloth configurations.

\input{tabs/abl_action_cond_table}

%% ── 3. Latent-Space Formulation ───────────────────────────────────────────────
\finding{\textbf{Latent-Space Choice.} A temporally-aware causal VAE ($4\times$ compression) outperforms a
frame-independent encoder on both InD and OoD, demonstrating that temporal context
in the latent space benefits even highly stochastic particle dynamics.}
The Wan~2.1 causal VAE applies $4\times$ temporal compression, coupling consecutive frames
in the latent space.
We ablate this against a frame-independent image VAE (FLUX VAE~\cite{flux2024}),
which encodes each frame independently ($1\times$ temporal compression).
Table~\ref{tab:abl_vae} reports results on Pour Water, a particle-dynamics environment
where per-frame spatial detail matters.
WanVAE outperforms FluxVAE on both InD (25.80\,dB vs.\ 24.89\,dB) and OoD
(24.57\,dB vs.\ 24.09\,dB), indicating that temporally-aware latent representations
are beneficial even for highly stochastic particle dynamics.

\input{tabs/abl_vae_table}

%% ── 4. Training Data Scaling ──────────────────────────────────────────────────
\finding{\textbf{Data Efficiency.} Data efficiency is governed by geometric variability: Pour Water degrades
gracefully with less data due to its single repeatable pouring motion, while
Push Cube degrades sharply as it requires diverse trajectory coverage over a wide workspace.}
We train DiT-S on Push Cube and Pour Water using 100\%, 50\%, and 25\% of the
available training trajectories (Table~\ref{tab:abl_data}).
Both environments show consistent monotonic degradation as data is reduced.
Push Cube degrades sharply (InD PSNR $-1.06$\,dB at 50\%, $-2.61$\,dB at 25\%),
indicating that diverse cube configurations and push directions require broad
trajectory coverage to generalize.
Pour Water is substantially more data-efficient: at 50\% data the InD drop is
only $-0.26$\,dB, and even at 25\% it retains reasonable performance ($-1.69$\,dB),
likely because its dynamics are governed by a single repeatable pouring motion
with limited geometric variability.

\input{tabs/abl_data_table}

%% ── 5. Action Dimensionality ──────────────────────────────────────────────────
\finding{\textbf{Action Dimensionality.} Richer action specifications disproportionately improve OoD generalization.
For Cloth Move, expanding from 3-DoF to 8-DoF per-arm actions dramatically boosts OoD
performance, as full per-arm descriptions help the model disentangle
manipulation intent from scene appearance.}
Table~\ref{tab:abl_actdim} examines whether a \textbf{higher-dimensional action space}
improves prediction accuracy.
For Cloth Move, we compare the reduced 3-DoF action ($\Delta x,\Delta y,\Delta z$
shared across both arms) used in the main benchmark against the full 8-DoF
per-arm action space.
For Push Cube, we compare a single pusher (action dim~2) against two independent
pushers (action dim~4), increasing both task complexity and the required
action-observation entanglement.
For Cloth Move, increasing the action space from 3-DoF (shared $\Delta xyz$) to 8-DoF
(per-arm $\Delta$pose $+$ grasp) dramatically improves OoD performance
($16.23\,\to\,21.60$\,dB, $+5.37$\,dB) at a modest InD cost ($-0.81$\,dB):
the full per-arm specification disambiguates arm motions and provides the model with
a richer conditioning signal that transfers better under distribution shift.
For Push Cube, the two-pusher variant represents a harder task with more complex
multi-object interactions; its larger OoD gap ($\Delta$PSNR $= -2.19$\,dB vs.\
$-0.05$\,dB for a single pusher) reflects the increased task difficulty
in addition to the higher-dimensional conditioning.

\input{tabs/abl_actdim_table}

WanVAE preserves finer water-surface texture and fill level across frames,
while FluxVAE produces smoother but less faithful fluid boundaries,
consistent with the quantitative gap in Table~\ref{tab:abl_vae}.

